A Privacy-Preserving Longevity Study of Tor's Hidden Services

Tor and hidden services have emerged as a practical solution to protect user privacy against tracking and censorship. At the same time, little is known about the lifetime and nature of hidden services. Data collection and study of Tor hidden services is challenging due to its nature of providing privacy. Studying the lifetime of hidden services provides several benefits. For example, it allows investigation of the maliciousness of domains based on their lifetime. Short-lived hidden services are more likely not to be legitimate domains, e.g., used by ransomware, as compared to long-lived domains. In this work, we investigate the lifetime of hidden services by collecting data from a small (2%) subset of all Tor HSDir relays in a privacy-preserving manner. Based on the data collected, we devise protocols and extrapolation techniques to infer the lifetime of hidden services. Moreover we show that, due to Tor's specifics, our small subset of HSDir relays is sufficient to extrapolate lifetime with high accuracy, while respecting Tor user and service privacy and following Tor's research safety guidelines. Our results indicate that a large majority of the hidden services have a very short lifetime. In particular, 50% of all current Tor hidden services have an estimate lifetime of only 10 days or less, and 80% have a lifetime of less than a month.

==> extrapolate.tex <==
\section{Extrapolation: Inferring Lifespan from the HSDir Counts}\label{s:extrapolate}

In this section, we review our approach to infer the lifespan of hidden services by extrapolating from the counts at the HSDirs. We use simulations by mimicking the process of the hidden service placing descriptors in the Tor network, according to the Tor's hidden service specification, to estimate the distribution of expected counts at HSDirs.


\subsection{Expected Counts at HSDirs}


If each hidden service was only placed on a single random HSDir, the
probability for each HSDir to host a hidden service is 
$p_0 = \frac{1}{N_{hsdirs}}$, where $N_{hsdirs}$ is the number of
HSDirs. The number of HSDirs is publicly available and can be found on the Tor's
 official metrics website. Since there are two descriptors, derived independently, this
is equivalent to doubling the number of potential hosting HSDirs. As each
descriptor is placed on a set of three adjacent HSDirs, the
probability of a descriptor being hosted on an HSDir is approximated by
$p \approx 6p_0 = \frac{6}{N_{hsdirs}}$. At the end of each 24 hour epoch, we would count each hidden service twice, because not all the hidden services change HSDirs at the same time. If a hidden service is online for $d$ days during our experiments, the average number of counts for a hidden service per HSDir relay, is as following.

\[C_h ^ d =\frac{6 \times d \times 2}{N_{hsdirs}}\] \\


In the above equation $C_h ^ d$ is the average expected count of hidden services $h$ that has been online for $d$ days during the experiment. Given that we control $N_{control}$ of the total HSDirs, the average total count for each hidden service ($C_h$), after $d$ days, from our HSDirs is outlined below.


\[ C_h ^ d =\frac{6 \times d \times 2 \times N_{control} }{N_{hsdirs}}\] \\


This formula gives us the average expected count values for each hidden service from our HSDirs. To calculate the distribution of the counts, we use simulations to find the expected observation counts as a function of the lifespan of a hidden service for the duration of the our study. Figure~\ref{f:expected_dist} shows the expected values for lifespan of hidden services. We calculate the mean, one standard deviation, two standard deviations and 95\% of the values from the mean value. The distribution of expected counts follows the bell curve distribution. As we can see, 95\% of the expected values are within two standard deviations of the mean expected value. 


\begin{figure}

\hspace{1cm}\includegraphics[width=0.45\textwidth]{graphs/extrapolate12_6months.pdf}
\caption{Expected counts at HSDirs as a function of lifespan. As we can see, 95\% of the expected values are within two standard deviation of the mean expected value.}
\label{f:expected_dist}
\end{figure}



Figure~\ref{f:expected_hists} depicts the histogram of expected values for different lifespans of 10 days, 30 days, 50 days, and 90 days. The results are based on 10000 runs of simulation. We simulate the placement of the descriptors on 6 relays according to Tor specifications for $d$ days. At the end of each run of the experiment, simulating a hidden service with lifespan $d$, we count the number of times that the descriptor is uploaded to the HSDirs under our control. The Y-axis, represents the frequency percentage for each expected count. As it is evident, the longer the lifespan of a hidden service, the closer its distribution of the counts to the bell curve distribution. As can be seen in Figure~\ref{f:10days_hist} (10 days) compared to Figure~\ref{f:90days_hist} (90 days). Moreover, the hidden services with shorter lifespan have a lower standard deviation and range of expected counts. This explains the large distribution of values around the expected counts of 1, 2, and 3.






\subsection{Weighted Frequency Count}

One approach to infer the lifespan of hidden services, is to use the mean expected count at HSDirs. However, this approach ignores all other possible expected counts, and certain values with higher probability of observation, dominate and skew the results. 


\begin{figure*}
     \centering
     \subfloat[][10 Days]{\includegraphics[width=0.45\textwidth]{graphs/10days_hist.pdf}\label{f:10days_hist}}
     \subfloat[][30 Days]{\includegraphics[width=0.45\textwidth]{graphs/30days_hist.pdf}\label{f:30days_hist}}\\
     \subfloat[][50 Days]{\includegraphics[width=0.45\textwidth]{graphs/50days_hist.pdf}\label{f:50days_hist}}
     \subfloat[][90 Days]{\includegraphics[width=0.45\textwidth]{graphs/90days_hist.pdf}\label{f:90days_hist}}
     \caption{Histograms of expected values for different lifespans, 10 days, 30 days, 50 days, and 90 days. The results are based on 10000 runs of simulation. The Y-axis, represents the frequency percentage for each expected count.}
     \label{f:expected_hists}
\end{figure*}

As shown in Figure~\ref{f:expected_dist}, 95\% of the counts are within the two standard deviations of the mean. By only using the mean value, majority of the expected counts are not accounted. For a better representative extrapolation of the lifespan, we use a weighted sum of the distribution of different longevities. For example, imagine for each lifespan $d_i$, we expect to have the count $x_{i,j}$ with probability $p_{i,j}$, $(x_{i,j}, p_{i,j})$. Then for each $x_{i, j}$, we count $p_{i,j}$ hidden services with lifespan of $d_i$ days. In this way, we compute a weighted inverse of the observed count.
 

